Search for dark matter produced in association with bottom or top quarks in $\sqrt{s}$ = 13 TeV pp collisions with the ATLAS detector

A search for weakly interacting massive particle dark matter produced in association with bottom or top quarks is presented. Final states containing third-generation quarks and missing transverse momentum are considered. The analysis uses 36.1 $fb^{-1}$ of proton-proton collision data recorded by the ATLAS experiment at $\sqrt{s}$ = 13 TeV in 2015 and 2016. No significant excess of events above the estimated backgrounds is observed. The results are interpreted in the framework of simplified models of spin-0 dark-matter mediators. For colour-neutral spin-0 mediators produced in association with top quarks and decaying into a pair of dark-matter particles, mediator masses below 50 GeV are excluded assuming a dark-matter candidate mass of 1 GeV and unitary couplings. For scalar and pseudoscalar mediators produced in association with bottom quarks, the search sets limits on the production cross-section of 300 times the predicted rate for mediators with masses between 10 and 50 GeV and assuming a dark-matter mass of 1 GeV and unitary coupling. Constraints on colour-charged scalar simplified models are also presented. Assuming a dark-matter particle mass of 35 GeV, mediator particles with mass below 1.1 TeV are excluded for couplings yielding a dark-matter relic density consistent with measurements.

==> acknowledgements/Makefile <==
# Makefile for creating ATLAS Acknowledegments

TEXLIVE  = 2016
PDFLATEX = pdflatex
BIBTEX   = biber

BASENAME = Acknowledgements-main

.PHONY: clean cleanpdf

run_pdflatex: $(BASENAME).pdf
	@echo "Made $<"

# Change TeX Live version
texlive: $(BASENAME).tex
	if [ $(TEXLIVE) -ge 2007 -a $(TEXLIVE) -lt 2100 ]; then \
	  echo "Changing texlive value in $<"; \
	  sed -i'.bak' 's/texlive=20[0-9][0-9]/texlive=$(TEXLIVE)/' $<; \
	else echo "Invalid value for TEXLIVE: $(TEXLIVE)"; fi; \

# Change biblatex backend
bibtex: $(BASENAME).tex
	if [ $(BIBTEX) = 'biber' -o $(BIBTEX) = 'bibtex' ]; then \
	  echo "Changing biblatex backend in $<"; \
	  sed -i'.bak' -e 's/backend=biber/backend=$(BIBTEX)/' -e 's/backend=bibtex/backend=$(BIBTEX)/' $<; \
	else echo "Invalid value for BIBTEX: $(BIBTEX)"; fi; \

# Standard LaTeX targets
$(BASENAME).pdf: $(BASENAME).tex
	$(PDFLATEX) $<
	-$(BIBTEX)  $(basename $<)
	$(PDFLATEX) $<
	$(PDFLATEX) $<

%.bbl: %.tex *.bib
	$(PDFLATEX) $*
	$(BIBTEX) $*

clean:
	-rm *.dvi *.toc *.aux *.log *.out *.blg *.bbl *.bcf *-blx.bib \
	 *.run.xml *.synctex.gz *~ *.fls *.fdb_latexmk .*.lb spellTmp 

cleanpdf:
	-rm $(BASENAME).pdf

cleanall: clean cleanpdf

